Equivariant division

Let C be a non-empty finite set, and Gamma a subgroup of the symmetric group S(C). Given a bijection f:A cross C to B cross C, the problem of Gamma-equivariant division is to find a quotient bijection h:A to B respecting whatever symmetries f may have under the action of S(A) cross S(B) cross Gamma. Say that Gamma is fully cancelling if this is possible for any f, and finitely cancelling if it is possible providing A,B are finite. Feldman and Propp showed that a permutation group is finitely cancelling just if it has a globally fixed point. We show here that a permutation group is fully cancelling just if it is trivial. This sheds light on the fact that all known division algorithms that eschew the Axiom of Choice depend on fixing an ordering for the elements of C.

==> equi_dot_bib <==
@article {fp,
    AUTHOR = {Feldman, David and Propp, James},
     TITLE = {Producing new bijections from old},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {113},
      YEAR = {1995},
     PAGES = {1--44}
}

@article {schwartz:fourA,
    AUTHOR = {Schwartz, Rich Evan},
     TITLE = {Pan [G]alactic [D]ivision},
   JOURNAL = {Math. Intelligencer},
  FJOURNAL = {The Mathematical Intelligencer},
    VOLUME = {37},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {8--10},
eprint={arXiv:1504.02179 [math.CO]},
note={\url{http://arxiv.org/abs/1504.02179}},
}

}

@book{hinkis,
author="Arie Hinkis",
title="Proofs of the Cantor-Bernstein Theorem: A Mathematical Excursion",
year="2013",
publisher="Birkhauser"
}



@misc{conwaydoyle:three,
title={Division by three},
author = {Peter G. Doyle and John Horton Conway},
year="1994",
eprint={arXiv:math/0605779 [math.LO]},
note={\url{http://arxiv.org/abs/math/0605779}},
}

@misc{doyleqiu:four,
title={Division by four},
author = {Peter G. Doyle and Cecil Qiu},
year="2015",
eprint={arXiv:math/1504.01402 [math.LO]},
note={\url{http://arxiv.org/abs/1504.01402}},
}

@book{bachmann:transfinite,
	author =	"H. Bachmann",
	title =		"Transfinite Zahlen (Zweite Auflage)",
	publisher =	"Springer",
	address =	"Berlin",
	year =		"1967"
}
@article{bernstein:mengenlehre,
	author =	"F. Bernstein",
	title =		"Untersuchungen aus der {M}engenlehre",
	journal =	"Math. Ann.",
	volume =	"61",
	year =		"1905",
	pages =		"117-154"
}
@article{garsiaMilne:rogers,
	author =	"A. M. Garsia and S. C. Milne",
	title =		"A {R}ogers-{R}amanujan bijection",
	journal =	"J. Combin. Theory, Series A",
	volume =	"31",
	year =		"1981",
	pages =		"289-339"
}
@book{jech:setTheory,
	author =	"T. Jech",
	title =		"Set Theory",
	publisher =	"Academic Press",
	address =	"New York",
	year =		"1978"
}

@article{lindenbaumTarski:ensembles,
	author =	"A. Lindenbaum and A. Tarski",
	title =		"Communication sur les recherches de la th\'{e}orie des ensembles",
	journal =	"Comptes Rendus des s\'{e}ances de la Soci\'{e}t\'{e} des Sciences et des Letters de Varsovie, Classe {I}{I}{I}",
	volume =	"19",
	year =		"1926",
	pages =		"299-330"
}

@book{nelson:predicative,
	author =	"E. Nelson",
	title =		"Predicative Arithmetic",
	publisher =	"Princeton University Press",
	address =	"Princeton",
	year =		"1986"
}

@article{remmel:partition,
	author =	"J. B. Remmel",
	title =		"Bijective proofs of some classical partition identities",
	journal =	"J. Combin. Theory, Series A",
	volume =	"33",
	year =		"1982",
	pages =		"273-286"
}

@article{sierpinski:two,
	author =	"W. Sierpinski",
	title =		"Sur l'\'{e}galit\'{e} $2m=2n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"3",
	year =		"1922",
	pages =		"1-6"
}

@article{sierpinski:leq,
	author =	"W. Sierpinski",
	title =		"Sur l'implication $2m\leq 2n \rightarrow m \leq n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"34",
	year =		"1947",
	pages =		"148-154"
}

@article{tarski:cancellation,
	author =	"A. Tarski",
	title =		"Cancellation laws in the arithmetic of cardinals",
	journal =	"Fundamenta Mathematica",
	volume =	"36",
	year =		"1949",
	pages =		"77-92"
}

@article{schwartz:four,
title={{P}an {G}alactic {D}ivision},
author = {Rich Schwartz},
journal={Math. Intell.},
volume={37},
number={3},
pages={8-10},
year={2015},
eprint={arXiv:1504.02179 [math.CO]},
note={\url{http://arxiv.org/abs/1504.02179}},
}

@book{hall:groups,
title={The Theory of Groups},
author={Marshall Hall},
year={1959}
}

@book {jech:choice,
    AUTHOR = {Jech, Thomas J.},
     TITLE = {The axiom of choice},
      YEAR = {1973}
}

